Time-Contrastive Learning Based Deep Bottleneck Features for Text-Dependent Speaker Verification

There are a number of studies about extraction of bottleneck (BN) features from deep neural networks (DNNs)trained to discriminate speakers, pass-phrases and triphone states for improving the performance of text-dependent speaker verification (TD-SV). However, a moderate success has been achieved. A recent study [1] presented a time contrastive learning (TCL) concept to explore the non-stationarity of brain signals for classification of brain states. Speech signals have similar non-stationarity property, and TCL further has the advantage of having no need for labeled data. We therefore present a TCL based BN feature extraction method. The method uniformly partitions each speech utterance in a training dataset into a predefined number of multi-frame segments. Each segment in an utterance corresponds to one class, and class labels are shared across utterances. DNNs are then trained to discriminate all speech frames among the classes to exploit the temporal structure of speech. In addition, we propose a segment-based unsupervised clustering algorithm to re-assign class labels to the segments. TD-SV experiments were conducted on the RedDots challenge database. The TCL-DNNs were trained using speech data of fixed pass-phrases that were excluded from the TD-SV evaluation set, so the learned features can be considered phrase-independent. We compare the performance of the proposed TCL bottleneck (BN) feature with those of short-time cepstral features and BN features extracted from DNNs discriminating speakers, pass-phrases, speaker+pass-phrase, as well as monophones whose labels and boundaries are generated by three different automatic speech recognition (ASR) systems. Experimental results show that the proposed TCL-BN outperforms cepstral features and speaker+pass-phrase discriminant BN features, and its performance is on par with those of ASR derived BN features. Moreover,....

==> References <==
@article{young2006htk,
  title={{T}he {HTK} {B}ook (v3. 4)},
  author={Young, S. and Evermann, G. and Gales, M. and Hain, T. and Kershaw, D. and Liu, X. and Moore, G. and Odell, J. and Ollason, D. and Povey, D. and others},
  journal={Cambridge University},
  year={2006}
}


@article{goroshin2015unsupervised,
  title={{U}nsupervised {F}eature {L}earning {F}rom {T}emporal {D}ata},
  author={Goroshin, R. and Bruna, J. and Tompson, J. and Eigen, D. and LeCun, Y.},
  journal={arXiv preprint arXiv:1504.02518},
  year={2015}
}

@inproceedings{mobahi2009deep,
  title={{D}eep {L}earning {F}rom {T}emporal {C}oherence in {V}ideo},
  author={Mobahi, H. and Collobert, R. and Weston, J.},
  booktitle={Proc. of the 26th Annual International Conference on Machine Learning},
  pages={737--744},
  year={2009},
  organization={ACM}
}

@inproceedings{hsu2017unsupervised,
  title={{U}nsupervised {L}earning {O}f {D}isentangled {A}nd {I}nterpretable {R}epresentations {F}rom {S}equential {D}ata},
  author={Hsu, W. -N. and Zhang, Y. and Glass, J.},
  booktitle={Advances in neural information processing systems},
  pages={1878--1889},
  year={2017}
}

@inproceedings{goodfellow2014generative,
  title={{G}enerative {A}dversarial {N}ets},
  author={Goodfellow, I. and Pouget-Abadie, J. and Mirza, M. and Xu, B. and Warde-Farley, D. and Ozair, S. and Courville, A. and Bengio, Y.},
  booktitle={{A}dvances in {N}eural {I}nformation {P}rocessing {S}ystems},
  pages={2672--2680},
  year={2014}
}

@article{kingma2013auto,
  title={{A}uto-encoding {V}ariational {B}ayes},
  author={Kingma, D. P. and Welling, M.},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{zhang2016understanding,
  title={{U}nderstanding {D}eep {L}earning {R}equires {R}ethinking {G}eneralization},
  author={Zhang, C. and Bengio, S. and Hardt, M. and Recht, B. and Vinyals, O.},
  journal={arXiv preprint arXiv:1611.03530},
  year={2016}
}

@inproceedings{zhang2016end,
  title={End-to-end {A}ttention {B}ased {T}ext-dependent {S}peaker {V}erification},
  author={Zhang, S. and Chen, Z. and Zhao, Y. and Li, J. and Gong, Y.},
  booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)},
  pages={171--178},
  year={2016}
  %organization={IEEE}
}

@inproceedings{geng2015multilingual,
  title={{M}ultilingual {T}andem {B}ottleneck {F}eature {F}or {L}anguage {I}dentification},
  author={Geng, W. and Li, J. and Zhang, S. and Cai, X. and Xu, B.},
  booktitle={Proc. of Interspeech},
  year={2015},
  pages={413--417}
}

@article{eskimez2018front,
  title={{F}ront-end {S}peech {E}nhancement {F}or {C}ommercial {S}peaker {V}erification {S}ystems},
  author={Eskimez, S. E. and Soufleris, P. and Duan, Z. and Heinzelman, W.},
  journal={Speech Communication},
  volume={99},
  pages={101--113},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{Li2018,
  author={N. Li and D. Tuo and D. Su and Z. Li and D. Yu},
  title={{D}eep {D}iscriminative {E}mbeddings {F}or {D}uration {R}obust {S}peaker {V}erification},
  year=2018,
  booktitle={Proc. of Interspeech},
  pages={2262--2266},
  doi={10.21437/Interspeech.2018-1769},
  url={http://dx.doi.org/10.21437/Interspeech.2018-1769}
}

@inproceedings{michelsanti2017conditional,
  title={{C}onditional {G}enerative {A}dversarial {N}etworks {F}or {S}peech {E}nhancement {A}nd {N}oise-{R}obust {S}peaker {V}erification},
  author={Michelsanti, D. and Tan, Z.-H.},
  booktitle={Proc. of Interspeech},
  pages={2008--2012},
  year={2017}
  %organization={ISCA}
}

@inproceedings{wang2018unsupervised,
  title={{U}nsupervised {D}omain {A}daptation {V}ia {D}omain {A}dversarial {T}raining {F}or {S}peaker {R}ecognition},
  author={Wang, Q. and Rao, W. and Sun, S. and Xie, L. and Chng, E. S. and Li, H.},
  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages={4889--4893},
  year={2018}
  %organization={IEEE}
}

@Article{Mahalanobis36,
	author={P. C. Mahalanobis},
	title={{O}n the {G}eneralised {D}istance in {S}tatistics},
	journal={Proc. of the National Institute of Sciences of India},
        volume={2},
	pages={49-55},
	year={1936}
}


@Article{MacQueen67,
	author={J. MacQueen},
	title={{S}ome {M}ethods for {C}lassification and {A}nalysis of {M}ultivariate {O}bservations},
	journal={Proc. of Fifth Berkeley Symp. on Math. Statist. and Prob. (Univ. of Calif. Press)},
	volume={1},
	pages={281-297},
	year={1967}
}

@Article{ross74,
	author={M. J. Ross and  H. L. Shaffer and A. Cohen and R. Freudberg and H. J.Manley},
	title={{A}verage {M}agnitude {D}ifference {F}unction {P}itch {E}xtractor},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={22},
	pages={353-362},
	year={1974}
}

@INPROCEEDINGS{Makhoul75,
	author = {J. Makhoul},
	title = {{L}inear {P}rediction: {A} {T}utorial {R}eview},
	booktitle = {Proceedings of the IEEE},
	volume={63},
	pages={561-580},
	year={1975}
}

@Article{Sambur76,
	author = {M. R. Sambur},
	title = {{S}peaker {R}ecognition using {O}rthogonal {L}inear {P}rediction},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={24},
	pages={283-289},
	year={1976}
}
	
@Article{Markel77,
	author = {J. D. Markel and B. T. Oshika and Jr. A. M. Gray},
	title = {{L}ong-term {F}eature {A}veraging for {S}peaker {R}ecognition},
        journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={25},
	pages={330-337},
	year={1977}
}

@Article{dempster77,
  author={A. Dempster and N. Laird and D. Rubin},
  title={{M}aximum {L}ikelihood {F}rom {I}ncomplete {D}ata {V}ia {EM} {A}lgorithm},
  journal={J. Roy. statist. Soc.},
  volume={39},
  pages={1-38},
  year={1977}
   }

@Article{Davis80,
	author={S. B. Davis and P. Mermelstein},
	title={{C}omparison of {P}arametric {R}epresentations for {M}onosyllabic {W}ord {R}ecognition {I}n {C}ontinuously {S}poken {S}entences},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={28},
	pages={357-366},
	year={1980}
}

@Article{LINDE80,
	author={Y. Linde and A. Buzo and  R. M. GRAY},
        title={{A}n {A}lgorithm for {V}ector {Q}uantizer {D}esign},
	journal={IEEE Trans. Communications},
	volume={28},
	pages={84-94},
	year={1980}
}

@Article{Furui81,
	author={S. Furui},
	title={{C}epstral {A}nalysis {T}echnique for {A}utomatic {S}peaker {V}erification},
	journal={IEEE Trans. on  Acoust. Speech Signal Processing},
	volume={29},
	pages={254-272},
	year={1981}
}

@Article{Rabiner89,
	author={L. R. Rabiner},
	title={{A} {T}utorial on {H}idden {M}arkov {M}odels and {S}elected {A}pplications in {S}peech {R}ecognition},
	journal={Proc. of the IEEE},
	volume={77},
	pages={257-285},
	year={1989}
}



@Article{Hermansky90,
	author={H. Hermansky},
	 title={{P}erceptual {L}inear {P}redictive ({PLP}) {A}nalysis {O}f {S}peech},
	 journal={J. Acoust. Soc. Am.},
	 volume={87},
	 pages={1738-1752},
	 year={1990}
}

@Article{Higgin91,
author="A. Higgins and L. Bahler and J. Porter",
title="{S}peaker {V}erification using {R}andomized {P}hrase {P}rompting",
journal="Digital Signal Processing",
volume="1",
 pages="89-106",
year="1991"	 
}

@INPROCEEDINGS{reynolds91,
	author = {D. A. Reynolds and L. P. Heck},
	title = {{I}ntegration of {S}peaker and {S}peech {R}ecognition {S}ystems},
         booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {869-872},
	year = {1991}
}


@INPROCEEDINGS{Rosenberg92,
	author = {A. E. Rosenberg and J. DeLong and C\-H Lee and B\-H Jaung and F. K. Soong},
	title = {{T}he {U}se of {C}ohort {N}ormalized {S}cores for {S}peaker {V}erification},
	booktitle = { Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {599-602},
	year = {1992}
}


@Article{Huang93,
author="X. Huang and K. Le",
title="{O}n {S}peaker-{I}ndependent, {S}peaker-{D}ependent, and {S}peaker- {A}daptive  {S}peech {R}ecognition",
journal="IEEE Trans. Speech Audio Proc.",
volume="1",
year="1993",
pages="150-157"
}   
@INPROCEEDINGS{Timit,
author = {J. S. Garofolo and L. F. Lamel and W. M. Fisher and J. G. Fiscus and  D. S. Pallett and N. L. Dahlgren and V. Zue},
title = {{TIMIT} {A}coustic-{P}honetic {C}ontinuous {S}peech {C}orpus {LDC}93{S}1},
publisher = {Web Download. Philadelphia: Linguistic Data Consortium},
year={1993}
}


@Article{Hermanksy94,
       author = {H. Hermanksy and N. Morgan},
       title = {{R}ASTA {P}rocessing of {S}peech},
       journal={IEEE Trans. on Speech and Audio Processing},
       volume={2},
       pages={578-589},
       year={1994}
}

@Article{Gauvain94,
	author = {J.-L. Gauvain and C.-H. Lee},
	title = {{M}aximum a {P}osteriori {E}stimation for {M}ultivariate {G}aussian {M}ixture {O}bservations of {M}arkov {C}hains},
	journal={IEEE Trans. on Speech and Audio Processing},
	volume={2},
	pages={291-298},
	 year={1994}
}


@Article{reynold95,
  author="D. A. Reynolds",
  title="{S}peaker {I}dentification and {V}erification {U}sing {G}aussian {M}ixture {S}peaker {M}odels",
  journal="Speech Communication",
  volume="17",
  pages="91-108",
  year="1995"
}

@Article{Leggeter95,
author="C. Leggetter and P. Woodland",
title="{M}aximum {L}ikelihood {L}inear {R}egression for {S}peaker {A}daptation of {H}MMs",
journal="Computer Speech and Language",
volume="9",
pages="171-186",
year="1995"	
}
@Article{Vapnik95,
	author={C. Cortes and V. Vapnik},
	title={{S}upport {V}ector {N}etworks},
	journal={Machine Learning},
	volume={20},
	pages={273-297},
	year={1995}
}

@INPROCEEDINGS{Talkin95,
	author = {D. Talkin},
        title = {{A} {R}obust {A}lgorithm for {P}itch {T}racking ({RAPT})},
	booktitle = {in Speech coding and synthesis (Elsevier, ed.)},
	pages = {495-518},
        year = {1995}
}

@INPROCEEDINGS{leerose96,
 author = {Li Lee and Richard C. Rose},
 title = {{S}peaker {N}ormalization using {E}fficient {E}requency {W}arping {P}rocedures},
 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {353-356},
 year = {1996}
}



@INPROCEEDINGS{Rosenberg96,
	 author = {A. E. Rosenberg and S. Parthasarathy},
	 title = {{S}peaker {b}ackground {m}odels for {c}onnected {d}igit {p}assword {s}peaker {V}erification},
	 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {81-84},
	 year = {1996}
}




@INPROCEEDINGS{LHeck97,
	  author = {L. Heck and M. Weintraub},
	  title = {{H}andset-dependent {B}ackground {M}odels for {R}obust {T}ext-{I}ndependent {S}peaker {R}ecognition},
          booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	  pages = {1071-1074},
	  year = {1997}
}


@INPROCEEDINGS{DET97,
	   author = {A. Martin and G. Doddington and T. Kamm and M. Ordowskiand and M. Przybocki},
	   title = {{T}he {DET} {C}urve {I}n {A}ssessment {O}f {D}etection {T}ask {P}erformance},
	   booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	   pages = {1895-1898},
	   year = {1997}
}  


@INPROCEEDINGS{Ariyaeeinia97,
	author= {A. M. Ariyaeeinia and P. Sivakumaran},
	title = {{A}nalysis and {C}omparison of {S}core {N}ormalization {M}ethods for {T}ext {D}ependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {1379-1382},
	year = {1997}
}


@article{Lee-Rose98,
      author="L. Lee and R. Rose",
      title="{F}requency {W}arping {A}pproach  to {S}peaker {N}ormalization",
      journal="IEEE Trans. on Speech and Audio Processing",
      volume={6},
      pages={49-59},
      year={1998}
}



@INPROCEEDINGS{reycls98,
	author= {D. A. Reynolds and et. al},
	title = {{B}lind {C}lustering of {S}peech {U}tterances {B}ased on {S}peaker and {L}anguage {C}haracteristics},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3193-3196},
	year={1998}
}

@INPROCEEDINGS{Hermansky98,
	author={S. Van Vuuren and H. Hermansky},
	title={{O}n the {I}mportance of {C}omponents of the {M}odulation {S}pectrum for {S}peaker {V}erification},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3205-3208},
	year = {1998}
}


@Article{Pellom98,
    author={B. L. Pellom and J. H. L. Hansen},
    title={{A}n {E}fficient {S}coring {A}lgorithm for {G}aussian {M}ixture {M}odel {B}ased {S}peaker {I}dentification},
    journal={IEEE Signal Proc. Lett.},
    volume={5},
    pages={281-284},
    year={1998}
}

@Article{HLDA98,
	author= {N. Kumar and A.G. Andreou},
	title={{H}eteroscedastic {D}iscriminant {A}nalysis and {R}educed {R}ank {HMMs} for {I}mproved {S}peech {R}ecognition},
	journal={Speech Communication},
	volume={26},
	pages={283-297},
	year={1998}
}

@INPROCEEDINGS{Isobe99,
	author= {T. Isobe and J. Takahashi},
	title = {{A} {N}ew {C}ohort {N}ormalization using {L}ocal {A}coustic {I}nformation for {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
        pages = {841-844},
	year={1999}
}

@INPROCEEDINGS{McLaugn99,
     author={J. McLaughlin and D. A. Reynolds and T. Gleason},
     title={{A} {S}tudy of {C}omputation {S}peed-ups of the {GMM-UBM} {S}peaker {R}ecognition {S}ystem},
     booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
     pages={1215-1218},
     year={1999}
}

@INPROCEEDINGS{Markowitz99,
	author={J. Markowitz},
       title={{I}eri and {O}ggi {D}omani: {S}peaker {R}ecognition {Y}esterday, {T}oday and tomorrow},
       booktitle = {Proc. of COST250 Workshop on Speacker Recognition in Telephony},
       year={1999}
}


@INPROCEEDINGS{Auckenthaler1999,
author={R. Auckenthaler and  E. Parris and  M. Carey},
title={{I}mproving a {GMM} {S}peaker {V}erification {S}ystem by {P}honetic {W}eighting},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages={313-316},
 year={1999}
}


@Article{kuhn2000,
author="R. Kuhn and J.-C. Junqua and P. Nguyen and N. Niedzielski",
title="{R}apid {S}peaker {A}daptation in {E}igenvoice {S}pace",
journal="IEEE Trans. on Speech and Audio Processing",
volume="8 (6)",
pages="695-707",
year="2000"	
}	  

@Article{reynold00,
  author="D. A. Reynolds and T. F. Quatieri and R. B. Dunn",
  title="{S}peaker {V}erification {U}sing {A}dapted {G}aussian {M}ixture {M}odels",
  journal="Digital Signal Processing",
  volume="10",
  pages="19-41",
 year="2000"	  
}

@Article{Tnorm00,
 author="R. Auckenthaler and M. Carey and H. Lloyd-Thomas",
 title="{S}core {N}ormalization for {T}ext-{I}ndependent {S}peaker {V}erification {S}ystem",
 journal="Digital Signal Processing",
 Volume="10",
 pages="42-54",
 year="2000"
 }


@INPROCEEDINGS{Wagner00,
     author= {D. Tran and M. Wagner},
     title = {{A} {P}roposed {L}ikelihood {T}ransformation for {S}peaker {V}erification},
     booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
     pages = {1069-1072},
     year={2000}
}


@Article{kishore00,
  author="S. P. Kishore and B. Yegnanarayana",
  title="{S}peaker {V}erification: {M}inimizing the {C}hannel {E}ffects using {A}utoassociative {N}eural {N}etwork {M}odels",
  journal="ICASSP",
  year="2000",
  pages="1101-1104"
}



@INPROCEEDINGS{Heck00,
	author= {R. Teunen and B. Shahshahani and L. Heck},
	title = {{A} {M}odel-based {T}ransformational {A}pproach to {R}obust {S}peaker {R}ecognition},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
        pages = {495-498},
        year={2000}
}

@INPROCEEDINGS{paliwal00,
	author= {B. Wildermoth and K. K. Paliwal},
	title = {{U}se of {V}oicing and {P}itch {I}nformation for {S}peaker {R}ecognition},
	booktitle = {Proc. 8th Australian Intern. Conf. Speech Science and Technology},
	pages = {324-328},
       year={2000}

}


@INPROCEEDINGS{Gadde2000,
	author= {V. R. R. Gadde},
	title = {{M}odeling {W}ord {D}uration},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {601-604},
        year={2000}
}

@INPROCEEDINGS{Wan2000,
	author= {V. Wan and W. M. Campbell},
	title = {{S}upport {V}ector {M}achines for {S}peaker {V}erification and {I}dentification},
	booktitle = {Proc. IEEE Signal Processing Society Workshop Neural Networks},
	pages = {775-784},
	year={2000}
}


@INPROCEEDINGS{Doddington2001,
        author= {G. Doddington},
        title = {{S}peaker {R}ecognition {B}ased on {I}diolectal {D}ifferences {B}etween {S}peakers},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {2521-2524},
        year={2001}
}  


@INPROCEEDINGS{Sturim01,
        author= {D. Sturim and D. A. Reynolds and E. Singer and J. P. Campbell},
        title = {{S}peaker {I}ndexing in {L}arge {A}udio {D}atabases using {A}nchor {M}odels},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {429-432},
        year={2001}
}

@INPROCEEDINGS{Auck01,
       author={R. Auckenthaler and J. S. Masion},
       title={{G}aussian {S}election {a}pplied to {T}ext-{I}ndependent {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={83-88},
       year={2001}
}

@INPROCEEDINGS{Pelecanos01,
       author={J. Pelecanos and S. Sridharan},
       title={{F}eature {W}arping for {R}obust {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={213-218},
       year= {2001}
}


@INPROCEEDINGS{Wang2001,
        author= {J. C. N. Wang and W. H. Tsai and L. S. Lee},
        title = {{E}igen-{MLLR} {C}oefficients as {N}ew {F}eature {P}arameters for {S}peaker {I}dentification},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {1385-1388},
        year={2001}
}


@INPROCEEDINGS{Kajarekar2001,
author= {S. Kajarekar and H. Hermansky},
title = {{S}peaker {V}erification {B}ased on {B}road {P}honetic {C}ategories},
booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
pages={201-206},
year={2001}
}

@INPROCEEDINGS{Glds_ker2002,
	author={W. M. Campbell},
	title={{G}eneralized {L}inear {D}iscriminant {S}equence {K}ernels for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {161-164},
	year={2002}
}


@INPROCEEDINGS{ReynoldsFmap,
	author= {D.A. Reynolds},
	title = {{C}hannel {R}obust {S}peaker {V}erification via {F}eature {M}apping},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {6-10},
        year={2003}
}


@INPROCEEDINGS{Tkinnun03,
    author={T. Kinnunen and E. Karpov and P. Franti},
    title={{A} {S}peaker {P}runing {A}lgorithm for {R}eal-{T}ime {S}peaker {I}dentification},
    booktitle = {Proc. Audio- and Video-Based Biometric Authentication},
    pages={639-646},
        year={2003}
}




@Article{nisteval04,
	author="{T}he {E}valuation {P}lan of NIST 2004 {S}peaker {R}ecognition {C}ampaign.
	http://www.itl.nist.gov/iad/mig//tests/sre/2004/SRE-04\_evalplan{-}v1a.pdf"
}

@INPROCEEDINGS{bonastre04,
        author = {J. F. Bonastre and N. Scheffer and C. Fredouille and D. Matrouf},
        title = {{N}IST'04 {S}peaker {R}ecognition {E}valuation {C}ampaign: {N}ew {LIA} {S}peaker {D}etection {P}lateform based on {ALIZE} {T}oolkit},
        booktitle = {Proc. of NIST 2004 Speaker Recognition Workshop},
        year = {2004},
}

@INPROCEEDINGS{Binma04,
	author = {B. Ma and H. Meng},
	title = {{E}nglish-{C}hinese {b}ilingual {t}ext-independent {s}peaker {v}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Leung04,
	author = {K. Y. Leung and M. W. Mak and S. Y. Kung},
	title = {{A}pplying {a}rticulatory {f}eatures to {t}elephone-based {s}peaker {v}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Kwong04,
	author = {Q.Y. Hong and S. Kwong},
	title = {{D}iscriminative {t}raining for {s}peaker {i}dentification based on {m}aximum {m}odel {d}istance {a}lgorithm},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}



@INPROCEEDINGS{Louradour05,
	author = {J. Louradour and K. Daoudi and R. Andre-Obrecht},
	title = {{D}iscriminative {P}ower of {T}ransient {F}rames in {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={613-616},
	year={2005}
}



@INPROCEEDINGS{Stolcke05,
	author= {A. Stolcke and L. Ferrer and S. Kajarekar and E. Shriberg and A. Venkataraman},
	title = {{MLLR} {T}ransforms as {F}eatures in {S}peaker {R}ecognition},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {2425-2428},
        year={2005}
}





@Article{kenny05,
author="P. Kenny",
title="{J}oint {F}actor {A}nalysis of {S}peaker and {S}ession {V}ariability : {T}heory and {A}lgorithms",
journal="Technical report CRIM-06/08-13  Montreal, CRIM",
year="2005"
}



@INPROCEEDINGS{AT_norm,
	author= {D. E. Sturim and D.A. Reynolds},
	title = {{S}peaker {A}daptive {C}ohort {S}election for {T}norm in {T}ext-independent {S}peaker {V}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {741-744},
        year={2005}
}	


@INPROCEEDINGS{datadriven05,
	author= {M. Mason and R. Vogt and B. Baker and S. Sridharan},
	title = {{D}ata-{D}riven {C}lustering for {B}lind {F}eature {M}apping in {S}peaker {V}erification},
	booktitle = {Proc. of Interspeech},
         pages = {3109-3112},
        year={2005}
}


@INPROCEEDINGS{ZTnorm05,
	author= {R. Vogt and B. Baker and S. Sridharan},
	title = {{M}odeling {S}ession {V}ariability in {T}ext-{I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {3117-3120},
	year={2005}
}

@INPROCEEDINGS{Adami05,
	author= {A. G. Adami},
        title = {{P}rosodic {M}odeling for {S}peaker {R}ecognition based on {S}ub-band {E}nergy {T}emporal {T}rajectories},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {189 - 192},
        year={2005}
}

@INPROCEEDINGS{NAP2005,
	author= {A. Solomonoff and W. M. Campbell and I. Boardman},
	title = {{A}dvances in {C}hannel {C}ompensation for {SVM} {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {629 - 632},
	year={2005}
}
@INPROCEEDINGS{Campbel_GMM_sup06,
author= {W. Campbell and D. Sturim and D. Reynolds and A. Solomonoff},
title = {{SVM} based {S}peaker {V}erification using a {GMM} {S}upervector {K}ernel and {NAP} {V}ariability {C}ompensation},
 booktitle = { Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {97-100},
 year={2006}
}

@INPROCEEDINGS{Goldberger05adistance,
author = {J. Goldberger and H. Aronowitz},
title = {{A} {D}istance {M}easure {B}etween {GMM}s {B}ased on the {U}nscented {T}ransform and its {A}pplication to {S}peaker {R}ecognition},
booktitle = {in Proc. of Interspeech},
pages = {1985-1989},
year = {2005}
}



@INPROCEEDINGS{krause06,
	author = {N. Krause and R. Gazit},
	title ={{SVM}-based {S}peaker {C}lassification in the {GMM} {M}odels {S}pace},
	booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	year ={2006}
}


@INPROCEEDINGS{Noor06,
	  author = { E. Noor and H. Aronowitz},
	  title={{E}fficient {L}anguage {I}dentification using {A}nchor {M}odels and {S}upport {V}ector {M}achines},    
	  booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	  year ={2006}
}



@INPROCEEDINGS{Binma06,
	author = {B. Ma and D. Zhu and R. Tong and H. Li},
	title={{S}peaker {C}luster {B}ased {GMM} {T}okenization for {S}peaker {R}ecognition},
	booktitle = {Proc. of Interspeech},
        year ={2006},
}


@INPROCEEDINGS{Hazen06,
  author="R. Woo and A. Park and T. J. Hazen",
  title="{T}he {MIT} {M}obile {D}evice {S}peaker {V}erification {C}orpus: {D}ata {C}ollection and {P}reliminary {E}xperiments",
  booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
  pages="1-6",
  year="2006"
}


@Article{Campbell2006,
	author={W. M. Campbell and D. E. Sturim and D. A. Reynolds},
	title={{S}upport {V}ector {M}achines using {GMM} {S}upervectors for {S}peaker {V}erification},
	 journal={IEEE Signal Process. Lett.},
	 volume={13},
	 pages={308-311},
	 year={2006}
}


@Article{Mami06,
	author="Y. Mami and D. Charlet",
	title="{S}peaker {R}ecognition by {L}ocation in the {S}pace of {R}eference {S}peakers",
	journal="Speech Communication",
	volume="48",
	pages="127-141",
	year="2006"
}

@Article{Skosan06,
	author={M. Skosan and D. Mashao},
	title={{M}odified {S}egmental {H}istogram {E}qualization for {R}obust {S}peaker {V}erification},
	journal={Pattern Recogn. Lett.},
        volume={27},
        pages={479–486},
        year={2006}
}	


@INPROCEEDINGS{hatch06,
   author = {A. Hatch and S. Kajarekar and A. Stolcke},
   title={{W}ithin-{C}lass {C}ovariance {N}ormalization for {SVM}-{B}ased {S}peaker {R}ecognition},
   booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
   pages = {1471-1474},
   year ={2006}
}


@INPROCEEDINGS{Guyon2006,
author="I. Guyon and A. Alamdari and G. Dror and J. Buhmann",
title="{P}erformance {P}rediction {C}hallenge",
booktitle ="Proc. of  IJCNN",
pages= "2958-2965",
year="2006"
}




@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} {B}ook",
  journal={Copyright 2001-2006 Cambridge University Engineering Department}
   }


@Article{Castro2007,
      author="D. R. Castro and et. al",
      title="{S}peaker {V}erification using {S}peaker- and {T}est-dependent {F}ast {S}core {N}ormalization",
      journal="Pattern Recogn. Lett.",
      volume="28",
      pages="90-98",
      year="2007"
}

@INPROCEEDINGS{Charbuillet07,
	author={C. Charbuillet and B. Gas and M. Chetouani and J. L. Zarader},
	title={{C}omplementary {F}eatures for {S}peaker {V}erification based on {G}enetic {A}lgorithms},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={285-288},
	year = {2007}
}

@INPROCEEDINGS{Xugang07,
	author={X. Lu and J. Dang},
	 title={{P}hysiological {F}eature {E}xtraction for {T}ext {I}ndependent {S}peaker {I}dentification using {N}on-{U}niform {S}ub-band {P}rocessing},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={461-464},
        year = {2007}
}

@INPROCEEDINGS{Saeidi07,
	author={R. Saeidi and H. R. Sadegh Mohammadi and R. D. Rodman and T. Kinnunen},
	title={{A} {N}ew {S}egmentation {A}lgorithm {C}ombined with {T}ransient {F}rames {P}ower for {T}ext {I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={305-308},
	year = {2007}
}
		
@INPROCEEDINGS{Tur2007,
	author={G. Tur and E. Shriberg and A. Stolcke and S. Kajarekar},
	title={{D}uration and {P}ronunciation {C}onditioned {L}exical {M}odeling for {S}peaker {S}erification},
        booktitle = {Proc. of Interspeech},
	pages={2049-2052},
	year = {2007}
}

@Article{HLDA_feat07,
	author={L. Burget and  P. Matejka and  O. Glembek and P. Schwarz and J. Cernocky},
        title = {{A}nalysis of {F}eature {E}xtraction and {C}hannel {C}ompensation in {GMM} {S}peaker {R}ecognition {S}ystem},
	journal={IEEE Trans. on Audio, Speech, Lang. Process.},
	volume={15},
	pages={1979-1986},
	year={2007}
}

@Article{fusion_2007,
	 author={N. Brummer and L. Burget and J. Cernocky and others},
	 title = {{F}usion of {H}eterogeneou {S}peaker {R}ecognition {S}ystems in the {STBU} {S}ubmission for the {NIST} {S}peaker {R}ecognition {E}valuation 2006},
	 journal={IEEE Trans. on Audio, Speech, and Lang. Process.},
	 volume={15},
	 pages={2072-2084},
	 year={2007}
}

@INPROCEEDINGS{Hazen97,
       author= {T. J. Hazen and J. R. Glass},
       title = {{A} {C}omparison of {N}ovel {T}echniques for {I}nstantaneous {S}peaker {A}daptation},
       booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
       pages = {2047-2050},
       year = {1997}
}


@INPROCEEDINGS{ferras-icassp08,
	author = {M. Ferras and  C. C. Leung and C. Barras and J. L. Gauvain},
        title = {{C}onstrained {MLLR} {F}or {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {53-56},
	year = {2007}
}


	       


@inproceedings{akhil-interspeech2008,
      author = {P. T. Akhil and S. P. Rath and S. Umesh and D. R. Sanand},
      title = {{A} {C}omputationally {E}fficient {A}pproach to {W}arp {F}actor {E}stimation in {VTLN} Using {EM} {A}lgorithm and {S}ufficient {S}tatistics},
      booktitle = {Proc. of Interspeech},
      pages = {1713-1716},
      year = {2008}
}


@inproceedings{sanand-interspeech2008,
      author={D. R. Sanand and S. Umesh},
      title={{S}tudy of {J}acobian {C}ompensation Using {L}inear {T}ransformation of {C}onventional {MFCC} for {VTLN}},
      booktitle={Proc. of Interspeech},
      pages={1233-1236},
      year={2008}
}

@Article{tsne,
author={L. J. P. van der Maaten and G. E. Hinton},
title={{V}isualizing {H}igh-{D}imensional {D}ata {U}sing {t-SNE}},
journal={Journal of Machine Learning Research},
volume={9},
pages={2579-2605},
year={2008}
}


@inproceedings{Yossi09,
	author = {Y. Bar-Yosef and Y. Bistritz},
        title = {{A}daptive {I}ndividual {B}ackground {M}odel for {S}peaker {V}erification},
        booktitle = {Proc. of Interspeech},
	pages = {1271-1274},
	year = {2009}
}	

@Article{Vraj09,
	author="V. R. Apsingekar and P. L. De Leon",
	title="{S}peaker {M}odel {C}lustering for {E}fficient {S}peaker {I}dentification in {L}arge {P}opulation {A}pplications",
	journal="IEEE Trans. on Speech and Language Processing",
	volume="17",
	pages="848-853",
	year="2009"
}

@inproceedings{Campbell2009,
author= {W. Campbell and Z. N. Karam}, 
title={{A} {F}ramework for {D}iscriminative {SVM GMM} {S}ystems for {L}anguage {R}ecognition},
booktitle = {Proc. of Interspeech},
year={2009}
}



@inproceedings{achintya-odyssey2010,
	author= {A. K. Sarkar and S. Umesh},
	title= {{I}nvestigation of {S}peaker-{C}lustered {UBM}s based on {V}ocal {T}ract {L}engths and {MLLR} matrices for {S}peaker {V}erification},
	booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	pages= {286-293},
	year = {2010}

}

@inproceedings{achintya-odyssey2010_spkid,
	      author= {A. K. Sarkar and S. Umesh and S. P. Rath},
	      title= {{C}omputationally {E}fficient {S}peaker {I}dentification for {L}arge {P}opulation {T}asks using {MLLR} and {S}ufficient {S}tatistics},
	      booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	      pages= {7-11},
              year = {2010}
}

@Article{Zheng_hua2010,
author={Z.-H. Tan and B. Lindbeg},
title={{L}ow-complexity {V}ariable {F}rame {R}ate {A}nalysis for {S}peech {R}ecognition and {V}oice {A}ctivity {D}etection},
journal={IEEE Journal of Selected Topics in Signal Processing},
volume={4},
pages={798- 807},
year={2010}
}

@inproceedings{Zhang-odyssey2010,
       author= {W. Q. Zhang and Y. Shan and J. Liu},
       title= {{M}ultiple {B}ackground {M}odels for {S}peaker {V}erification},
       booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={47-51},
       year = {2010}
}


@inproceedings{achintya-inter2010,
             author= {A. K. Sarkar and S. Umesh},
             title= {{F}ast {C}omputation of {S}peaker {C}haracterization {V}ector using {MLLR} and {S}ufficient {S}tatistics in {A}nchor {M}odel {F}ramework},
             booktitle = {Proc. of Interspeech},
	     pages={2738-2741},
	     year = {2010}
}

@Article{Kinnunen2010,
author={T.  Kinnunen  and  H.  Li},
title={{A}n  {O}verview  {O}f  {T}ext-independent {S}peaker {R}ecognition:  {F}rom {F}eatures {T}o {S}upervectors},
journal={Speech Communication},
volume={52},
pages={12-40},
year={2010}
}

@Article{Zheng-Hua2010,
author={Z.-H. Tan and B. Lindber},
title={{L}ow-{C}omplexity {V}ariable {F}rame {R}ate {A}nalysis for {S}peech {R}ecognition and {V}oice {A}ctivity {D}etection},
journal={IEEE Journal of Selected Topics in Signal Processing},
volume={4},
pages={798-807},
year={2010}
}




@inproceedings{achintya-icassp2011,
	        author= {A. K. Sarkar and S. Umesh},
	        title= {{U}se of {VTL}-wise {M}odels in {F}eature-{M}apping {F}ramework {T}o {A}chieve {P}erformance of {M}ultiple-{B}ackground {M}odels in {S}peaker {V}erification},
	        booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
		pages={4552-4555},
	        year = {2011}

}

@Article{Deka_ieee2011,
       author= {N. Dehak and P. Kenny and R. Dehak and P. Ouellet and P. Dumouchel},
       title= {{F}ront-{E}nd {F}actor {A}nalysis {F}or {S}peaker {V}erification},
       journal={IEEE Trans. on Audio, Speech and Language Processing},
       volume={19},
       pages={788-798},
       year = {2011}
}

@inproceedings{Romero2011,
        author= {D. G. Romero and C. Y. Espy-Wilson},
        title= {{A}nalysis of i-vector {L}ength {N}ormalization in {S}peaker {R}ecognition {S}ystems},
        booktitle={Proc. of Interspeech},
        pages={249-252},
        year={2011}
}

@inproceedings{Kanagasundaram2011,
author={A. Kanagasundaram and R. Vogt and D. Dean and  S. Sridharan and M. Mason},
title= {i-vector based {S}peaker {R}ecognition on {S}hort {U}tterances},
booktitle={Proc. of Interspeech},
pages={2341-2344},
year={2011}
}


@inproceedings{SenoussaouiInterspch2011,
        author= {M. Senoussaoui and others},
        title= {{M}ixture of {PLDA} {M}odels {I}n {I}-{V}ector {S}pace {F}or {G}ender-{I}ndependent {S}peaker {R}ecognition},
        booktitle={Proc. of Interspeech},
        pages={25-28},
         year = {2011}
}


@inproceedings{Pierre-interspeech2012,
       author= {P. M. Bousquet and others},
       title= {{V}ariance-{S}pectra {B}ased {N}ormalization {F}or i-vector {S}tandard {A}nd {P}robabilistic {L}inear {D}iscriminant {A}nal
ysis},
       booktitle={Proc. of  Odyssey Speaker and Language Recognition Workshop},
       year={2012}
}


@inproceedings{Prince2012,
        author= {S. J. D. Prince},
        title= {{C}omputer {V}ision: {M}odels {L}earning {A}nd {I}nference},
        booktitle={Cambridge University Press, 1e, 2012}
}

@inproceedings{Larcher2012,
author= {A. Larcher and K. A. Lee and  B. Ma and H. Li},
title= {{RSR2015}: {D}atabase for {T}ext-dependent {S}peaker {V}erification using {M}ultiple {P}ass-phrases},
booktitle={Proc. of Interspeech},
pages={1580-1583},
 year = {2012}
}

@inproceedings{achintya2012,
author={A. K. Sarkar and  D. Matrouf and P. M. Bousquet and J. F. Bonastre},
title= {{S}tudy of the {E}ffect of i-vector {M}odeling on {S}hort and {M}ismatch {U}tterance {D}uration for {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={2662-2665},
year={2012}
}

@inproceedings{bob2012,
  author = {A. Anjos and L. El Shafey and R. Wallace and  M. G\"unther AND C. McCool AND S. Marcel},
  title = {Bob: {A} {F}ree {S}ignal {P}rocessing and {M}achine {L}earning {T}oolbox for {R}esearchers},
  year = {2012},
  month = oct,
  booktitle = {20th ACM Conference on Multimedia Systems (ACMMM), Nara, Japan},
  publisher = {ACM Press}
}

@inproceedings{Hinton2012,
author = {G. Hinton and others},
title = {{D}eep {N}eural {N}etworks {F}or {A}coustic {M}odeling {I}n {S}peech {R}ecognition},
booktitle={IEEE Signal Process. Mag.},
pages={82-97},
year={2012}
}


@Article{Dahl2012,
author={ E. Dahl and D. Yu and L. Deng and and A. Acero},
title = {{C}ontext-dependent {P}re-trained {D}eep {N}eural {N}etworks for {L}arge {V}ocabulary {S}peech {R}ecognition},
journal={IEEE Transactions on Audio, Speech, and Language Processing},
volume={20},
pages={30-42},
year={2012}
}



@inproceedings{Cong-Thanh2013,
author = {C.-T. Do and C. Barras and V.-B. Le and A. K. Sarkar},
title = {{A}ugmenting {S}hort-term {C}epstral {F}eatures {W}ith {L}ong-term {D}iscriminative {F}eatures {F}or {S}peaker {V}erification {O}f {T}elephone {D}ata},
booktitle={Proc. of Interspeech},
pages={2484-2488},
year={2013}
}


@inproceedings{Fu2014,
author={T. Fu and Y. Qian and Y. Liu and Kai Yu}, 
title= {{T}andem {D}eep {F}eatures {F}or {T}ext-dependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1327-1331},
year = {2014}
}

@article{DBLP:journals/spl/SarkarDLB14,
  author    = {A. K. Sarkar and C. T. Do and V. B. Le and
               C. Barras},
  title     = {{C}ombination {O}f {C}epstral {A}nd {P}honetically {D}iscriminative {F}eatures {F}or {S}peaker {V}erification},
  journal   = {{IEEE} Signal Process. Lett.},
  volume    = {21},
  number    = {9},
  pages     = {1040--1044},
  year      = {2014},
  }


@inproceedings{Kenny2014,
author={P. Kenny and V. Gupta and T. Stafylakis and P. Ouellet and J. Alam},
title= {{D}eep {N}eural {N}etworks for {E}xtracting {B}aum-welch {S}tatistics for {S}peaker {R}ecognition},
booktitle={Proc. of  Odyssey Speaker and Language Recognition Workshop},
pages={293-298},
year = {2014}
}


@inproceedings{Nicolas2014,
author={N. Scheffer and Y. Lei},
title= {{C}ontent {M}atching for {S}hort {D}uration {S}peaker {R}ecognition},
booktitle={Proc. of Interspeech},
pages={1317-1321},
year = {2014}
}

@inproceedings{Hagai2014,
author={H. Aronowitz and  A. Rendel},
title= {{D}omain {A}daptation for {T}ext {D}ependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1337-1341},
year = {2014}
}

@inproceedings{Khoury2014,
author={E. Khoury and T. Kinnunen and  A. Sizov and Z. Wu and S. Marcel},
title={{I}ntroducing {I}-Vectors for {J}oint {A}nti-{S}poofing and {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={ 61-65},
year ={2014}
}

@inproceedings{Variani2014,
author={E. Variani and X. Lei and E. McDermott and I. Lopez-Moreno and J. Gonzalez-Dominguez},
title={{D}eep {N}eural {N}etworks {F}or {S}mall {F}ootprint {T}ext-dependent {S}peaker {V}erification},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages={4080-4084},
year ={2014}
}

@misc{Zhizheng2014,
author={Z. Wu and T. Kinnunen and N. Evans and J. Yamagishi},
title={{ASV}spoof {2015}: {A}utomatic {S}peaker {V}erification {S}poofing and {C}ountermeasures {C}hallenge {E}valuation {P}lan},
year ={2014}
}

@inproceedings{Yaman2012,
author={S. Yaman and J. Pelecanos and R. Sarikaya},
title={{B}ottleneck {F}eatures {F}or {S}peaker {R}ecognition},
booktitle={Odyssey},
year={2012},
pages={105-108}
}


@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent {S}peaker {V}erification: {C}lassifiers, {D}atabases and {RSR2015}},
journal={Speech Communication},
volume={60},
pages={56-77},
year={2014}
}

@inproceedings{Sahidullah2015,
author={M. Sahidullah  and T. Kinnunen and C. Hanilci},
title={{A} {C}omparison of {F}eatures for {S}ynthetic {S}peech {D}etection},
booktitle={in Proc. of Interspeech},
year={2015}
}


@Article{Yuan2015,
author={Y. Liu and Y. Qian and N. Chen and T. Fu and Y. Zhang and K. Yu},
title= {{D}eep {F}eature {F}or {T}ext-dependent {S}peaker {V}erification},
journal={Speech Communication},
volume={73},
pages={1-13},
year={2015}
}

@inproceedings{Ghalehjegh2015,
author={S. Ghalehjegh and R. Rose},
title= {{D}eep {B}ottleneck {F}eatures {F}or i-vector {B}ased {T}ext-independent {S}peaker {V}erification},
booktitle={Proc. of  IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)},
pages={555-560},
year={2015}
}


@inproceedings{McLaren2015,
author={M. McLaren and Y. Lei and L. Ferrer},
title={{A}dvances {I}n {D}eep {N}eural {N}etwork {A}pproaches {T}o {S}peaker {R}ecognition},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2015}
}




@inproceedings{achintya2016,
author={A. K. Sarkar and Z.-H. Tan},
title={{T}ext {D}ependent {S}peaker {V}erification Using {U}nsuper-vised {HMM-UBM} and {T}emporal {GMM-UBM}},
booktitle={Proc. of Interspeech},
year={2016}
}

@inproceedings{Kinnunen2016,
author={T. Kinnunen and M. Sahidullah and I. Kukanov and H. Delgado and M. Todisco and A. Sarkar and N. Bæk Thomsen and V. Hautamaki and N. Evans and Z.-H. Tan},
title={{U}tterance {V}erification {F}or {T}ext-dependent {S}peaker {R}ecognition: {A} {C}omparative {A}ssessment {U}sing {T}he {R}ed{D}ots {C}orpus},
booktitle={Proc. of Interspeech},
year={2016}
}


@inproceedings{Yu2016,
author={H. Yu and A. Sarkar and D. A. L. Thomsen and Z. H. Tan and  Z. Ma and J. Guo},
title={{E}ffect of {M}ulti-condition {T}raining and {S}peech {E}nhancement {M}ethods {O}n {S}poofing {D}etection},
booktitle={Proc. of  International Workshop on Sensing, Processing and Learning for Intelligent Machines (SPLINE)},
pages={1-5},
year={2016}
}

@inproceedings{Sahidullah_ASV_spoof2016,
author={M. Sahidullah and H. Delgad amd  M. Todisco and H. Yu and T. Kinnunen and N. Evans and  Z.-H. Tan},
title={{I}ntegrated {S}poofing {C}ountermeasures and {A}utomatic {S}peaker {V}erification: {A}n {E}valuation on {ASV}spoof 2015},
booktitle={in Proc. of Interspeech},
pages={1700-1704},
year={2016}
}


@inproceedings{Aapo2016,
author={A. Hyvarinen and H. Morioka},
title={{U}nsupervised {F}eature {E}xtraction {b}y {T}ime-{C}ontrastive {L}earning {A}nd {N}onlinear {ICA}},
booktitle={Proc. of Neural Information Processing systems (NIPS)},
year={2016}
}


@inproceedings{Delgado2016Asru,
author={H. Delgado and  M. Todisco and  M. Sahidullah and  A. K. Sarkar and N. Evans and  T. Kinnunen and  Z.-H. Tan},
title={{F}URTHER {O}PTIMISATIONS OF {C}ONSTANT {Q} {C}EPSTRAL {P}ROCESSING {F}OR {I}NTEGRATED {U}TTERANCE {A}ND {T}EXT-DEPENDENT {S}PEAKER {V}ERIFICATION},
booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)},
year={2016}
}

@Article{alizetoolkit,
  title="http://lia.univ-avignon.fr/heberges/ALIZE/"
   }

@Article{mit_database,
  title="http://groups.csail.mit.edu/sls/mdsvc"
}

@Book{duda_hart_patt,
	  author = {R.O. Duda and P.E. Hart and D.G. Stork},
	  title  = {{P}attern {C}lassification},
	  publisher = {New York: John Wiley \& Sons},
	  year    = {2001}
}


@misc{Focal,
	author= {N. Brummer},
	title= {{F}oCal {T}oolkit},
	 howpublished ={Available at http://sites.google.com/site/nikobrummer/focal}
}

@misc{Lnknet,
title= {http://www.ll.mit.edu/mission/communications/ist/lnknet/index.html}
}
@misc{RedDots,
title= {{T}he {R}edDots {C}hallenge: {T}owards {C}haracterizing {S}peakers {F}rom {S}hort {U}tterances},
howpublished ={https://sites.google.com/site/thereddotsproject/reddots-challenge}
}

@misc{CNTK,
author= {A. Agarwal and others},
title= {{A}n {I}ntroduction to {C}omputational {N}etworks and the {C}omputational {N}etwork {T}oolkit},
year={2016}
}
howpublished ={https://www.microsoft.com/en-us/research/publication/an-introduction-to-computational-networks-and-the-computational-network-toolkit/


@inproceedings{AchintyaNips2017,
author={A. K. Sarkar and Z.-H. Tan},
title={{T}ime-{C}ontrastive {L}earning {B}ased {DNN} {B}ottleneck {F}eatures  {F}or {T}ext-{D}ependent {S}peaker {V}erification},
booktitle={Neural Information Processing systems (NIPS) Time Series Workshop},
year={2017}
}

@inproceedings{Schwarz,
author = {Schwarz, P. and Matejka, P. and Cernocky, J.},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
doi = {10.1109/ICASSP.2006.1660023},
isbn = {1-4244-0469-X},
mendeley-groups = {[bib]{\_}for{\_}paper/odyssey2018{\_}interspeech},
pages = {325--328},
title = {{H}ierarchical {S}tructures of {N}eural {N}etworks for {P}honeme {R}ecognition},
url = {http://ieeexplore.ieee.org/document/1660023/},
year = {2006}
}

@inproceedings{mclaren2015advances,
  title={{A}dvances {I}n {D}eep {N}eural {N}etwork {A}pproaches {T}o {S}peaker {R}ecognition},
  author={McLaren, M. and Lei, Y. and Ferrer, L.},
  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages={4814--4818},
  year={2015}
  }

@article{michelsanti2017conditional,
  title={{C}onditional {G}enerative {A}dversarial {N}etworks for {S}peech {E}nhancement and {N}oise-{R}obust {S}peaker {V}erification},
  author={Michelsanti, D. and Tan, Z.-H.},
  journal={Proc. of Interspeech 2017},
  pages={2008--2012},
  year={2017}
}


@inproceedings{variani2014deep,
  title={{D}eep {N}eural {N}etworks for {S}mall {F}ootprint {T}ext-dependent {S}peaker {V}erification},
  author={Variani, E. and Lei, X. and McDermott, E. and Moreno, I. L. and Gonzalez-Dominguez, J.},
  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages={4052-4056},
  year={2014}
  }

@inproceedings{yu2017adversarial,
  title={{A}dversarial {N}etwork {B}ottleneck {F}eatures {F}or {N}oise {R}obust {S}peaker {V}erification},
  author={Yu, H. and Tan, Z.-H. and Ma, Z. and Guo, J.},
  booktitle={Proc. of Interspeech},
  pages={1492--1496},
  year={2017}
}

@article{sarkar2018incorporating,
  title={{I}ncorporating {P}ass-phrase {D}ependent {B}ackground {M}odels {F}or {T}ext-dependent {S}peaker {V}erification},
  author={Sarkar, A. K. and Tan, Z.-H.},
  journal={Computer Speech \& Language},
  volume={47},
  pages={259--271},
  year={2018},
  publisher={Elsevier}
}

@article{tang2017endtoend,
  title = {{E}nd-to-End {N}eural {S}egmental {M}odels {F}or {S}peech {R}ecognition},
  author = {H. Tang and L. Lu and K. Gimpel and K. Livescu and C. Dyer and N. A. Smith and S. Renals},
  year = {2017},
  pages={1254-1264},
  journal = {IEEE Journal of Selected Topics in Signal Processing},
  volume = {11}
}

@phdthesis{tang2017sequence,
  title = {{S}equence {P}rediction {W}ith {N}eural {S}egmental {M}odels},
  author = {H. Tang},
  school = {Toyota Technological Institute at Chicago},
  year = {2017}
}

@inproceedings{tang2016endtoend,
  title = {{E}nd-to-end {T}raining {A}pproaches {F}or {D}iscriminative {S}egmental {M}odels},
  author = {H. Tang and W. Wang and K. Gimpel and K. Livescu},
  year = {2016},
  booktitle = {Proc. of  IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)}
}


@inproceedings{harwath2016unsupervised,
  title={{U}nsupervised {L}earning {O}f {S}poken {L}anguage {W}ith {V}isual {C}ontext},
  author={Harwath, D. and Torralba, A. and Glass, J.},
  booktitle={Proc. of Neural Information Processing systems (NIPS) },
  year={2016}
}

@article{kinnunen2010overview,
  title={{A}n {O}verview {O}f {T}ext-independent {S}peaker {R}ecognition: {F}rom {F}eatures {T}o {S}upervectors},
  author={Kinnunen, T. and Li, H.},
  journal={Speech communication},
  volume={52},
  number={1},
  pages={12--40},
  year={2010}
 }

@inproceedings{lee2015reddots,
  title={{T}he {R}edDots {D}ata {C}ollection {F}or {S}peaker {R}ecognition},
  author={Lee, K. A. and Larcher, A. and Wang, G. and Kenny, P. and Br{\"u}mmer, N. and Leeuwen, D. V. and Aronowitz, H. and Kockmann, M. and Vaquero, C. and Ma, B. and others},
  booktitle={Proc. of Interspeech},
  pages={2996-3000},
  year={2015}
}

@inproceedings{Aapo2016,
author={A. Hyvarinen and H. Morioka},
title={{U}nsupervised {F}eature {E}xtraction by {T}ime-{C}ontrastive {L}earning and {N}onlinear {ICA}},
booktitle={Proc. of Neural Information Processing systems (NIPS)},
year={2016}
}

@article{yu2014introduction,
  title={{A}n {I}ntroduction to {C}omputational {N}etworks {A}nd {T}he {C}omputational {N}etwork {T}oolkit},
  author={Yu, D. and Eversole, A. and Seltzer, M. and Yao, K. and Huang, Z. and Guenter, B. and Kuchaiev, O. and Zhang, Y. and Seide, F. and Wang, H. and others},
  journal={Microsoft Technical Report MSR-TR-2014--112},
  year={2014}
}




@inproceedings{Shi2018,
  author={Z. Shi and H. Lin and L. Liu and R. Liu},
  title={{L}atent {F}actor {A}nalysis of {D}eep {B}ottleneck {F}eatures {F}or {S}peaker {V}erification   {w}ith {R}andom {D}igit {S}trings},
  year=2018,
  booktitle={Proc. of Interspeech},
  pages={1081--1085},
   
}

@inproceedings{DBLP:conf/asru/ChenLXML17,
  author    = {H. Chen and C.{-}C. Leung and L. Xie and B. Ma and H. Li},
  title     = {{M}ultilingual {B}ottle-neck {F}eature {L}earning {F}rom {U}ntranscribed {S}peech},
  booktitle = {Proc. of  IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)},
  pages     = {727--733},
  year      = {2017}
 }
 
@inproceedings{DBLP:conf/asru/CYuan17,
author={Y. Yuan and C.-C. Leung and L. Xie and H. Chen and B. Ma and H. Li},
title={{E}xtracting {B}ottleneck {F}eatures {A}nd {W}ord-like {P}airs {F}rom {U}ntranscribed {S}peech {F}or {F}eature {R}epresentation},
booktitle = {Proc. of  IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)},
 pages={734-739},
 year={2017}
 }

@inproceedings{DBLP:conf/interspeech/LiMBPD16,
  author    = {R. Li and S. H. R. Mallidi and L. Burget and O. Plchot and             N. Dehak},
  title     = {{E}xploiting {H}idden-Layer {R}esponses {O}f {D}eep {N}eural {N}etworks {F}or {L}anguage  {R}ecognition},
  booktitle = {Proc. of Interspeech},
  pages     = {3265--3269},
  year      = {2016}
}

@inproceedings{DBLP:conf/interspeech/RichardsonRD15,
  author    = {F. Richardson and D. A. Reynolds and N. Dehak},
  title     = {{A} {U}nified {D}eep {N}eural {N}etwork {F}or {S}peaker and {L}anguage {R}ecognition},
  booktitle = {Proc. of Interspeech}
  pages     = {1146--1150},
  year      = {2015}
  }
@inproceedings{McLaren2016,
author={M. McLaren and L. Ferrer and A. Lawson},
title={{E}xploring the {R}ole of {P}honetic {B}}ottleneck {F}eatures for {S}peaker and {L}anguage {R}ecognition},
 booktitle ={Proc of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 year={2016}
 }
 
 @article{Radek17,
 author={R. Fer and P. Matejka and F. Grezl and O. Plchot and K. Vesely and J. H. Cernocky},
 title={{M}ultilingually {T}rained {B}ottleneck {F}eatures {I}n {S}poken {L}anguage {R}ecognition},
 Journal={Computer Speech \& Language},
 volume={46},
 year={2017},
 pages={252-267}
 }

@inproceedings{Ranjan2017,
  author={S. Ranjan and J. H.L. Hansen},
  title={{I}mproved {G}ender {I}ndependent {S}peaker {R}ecognition {U}sing {C}onvolutional {N}eural {N}etwork {B}ased {B}ottleneck {F}eatures},
  year=2017,
  booktitle={Proc. of Interspeech},
  pages={1009--1013},
  
}






